The Aizenman-Sims-Starr and Guerra's schemes for the SK model with multidimensional spins

We prove upper and lower bounds on the free energy in the Sherrington-Kirkpatrick model with multidimensional (e.g., Heisenberg) spins in terms of the variational inequalities based on the corresponding Parisi functional. We employ the comparison scheme of Aizenman, Sims and Starr and the one of Guerra involving the generalised random energy model-inspired processes and Ruelle's probability cascades. For this purpose an abstract quenched large deviations principle of the Gaertner-Ellis type is obtained. Using the properties of Ruelle's probability cascades and the Bolthausen-Sznitman coalescent, we derive Talagrand's representation of the Guerra remainder term for our model. We study the properties of the multidimensional Parisi functional by establishing a link with a certain class of the non-linear partial differential equations. Solving a problem posed by Talagrand, we show the strict convexity of the local Parisi functional. We prove the Parisi formula for the local free energy in the case of the multidimensional Gaussian a priori distribution of spins using Talagrand's methodology of the a priori estimates.

==> cupdef.tex <==
 \def\dist{d_N}
\def\phii{I}
\def\a{\alpha}
\def\b{\beta}
\def\d{\delta}
\def\e{\epsilon}
\def\ve{\varepsilon}
\def\f{\phi}
\def\g{\gamma}
\def\k{\kappa}
\def\l{\lambda}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
\def\th{\theta}
\def\vt{\vartheta}
\def\vp{\varphi}
\def\z{\zeta}
\def\o{\omega}
\def\D{\Delta}
\def\L{\Lambda}
\def\G{\Gamma}
\def\O{\Omega}
\def\S{\Sigma}
\def\Th{\Theta}
\def\del #1{\frac{\partial^{#1}}{\partial\l^{#1}}}

\def\h{\eta}

\def\1{{1\kern-.25em\rm{I}}}
\def\eu{{1\kern-.25em\rm{I}}}
\def\f1{{1\kern-.25em\rm{I}}}
\def\R{{\Bbb R}}  %%
\def\N{{\Bbb N}}  %%  
\def\P{{\Bbb P}}  %% carateri piu belle per campi di nombre  
\def\Z{{\Bbb Z}}  %% 
\def\Q{{\Bbb Q}}  %%
\def\C{{\Bbb C}}  %%
\def\DDD{{\Bbb D}}  %%
\def\E{{\Bbb E}}  %%
\def\M{{\Bbb M}}  %%
\def\U{{\Bbb U}}
\def\Va{{\Bbb V}}  %%
\def\T{{\Bbb T}}

\def\cs{{\check \s}}


\def\la{\langle}
\def\ra{\rangle} 
\def\der{\frac{d}{dx}}
\def\del{\partial}
\def\tr{\rm{tr}}
\def\dist{\,\rm{dist}}
\def\pb{\Phi_\b}
\let\cal=\Cal

\def\AA{{\mathcal A}}
\def\BB{{\mathcal B}}
\def\CC{{\mathcal C}}
\def\DD{{\mathcal D}}
\def\EE{{\mathcal E}}
\def\FF{{\mathcal F}}
\def\GG{{\mathcal G}}
\def\HH{{\mathcal H}}
\def\II{{\mathcal I}}
\def\JJ{{\mathcal J}}
\def\KK{{\mathcal K}}
\def\LL{{\mathcal L}}
\def\MM{{\mathcal M}}
\def\NN{{\mathcal N}}
\def\OO{{\mathcal O}}
\def\PP{{\mathcal P}}
\def\QQ{{\mathcal Q}}
\def\RR{{\mathcal R}}
\def\SS{{\mathcal S}}
\def\TT{{\mathcal T}}
\def\VV{{\mathcal V}}
\def\UU{{\mathcal U}}
\def\VV{{\mathcal V}}
\def\WW{{\mathcal W}}
\def\XX{{\mathcal X}}
\def\YY{{\mathcal Y}}
\def\ZZ{{\mathcal Z}}
\def\A{{\mathcal A}}

\def\chap #1#2{\line{\ch #1\hfill}\numsec=#2\numfor=1\numtheo=1}
\def\sign{\,\rm{sign}\,}
\def\un #1{\underline{#1}}
\def\ov #1{\overline{#1}}
\def\ba{{\backslash}}
\def\sb{{\subset}}
\def\wt{\widetilde}
\def\wh{\widehat}
\def\sp{{\supset}}
\def\rar{{\rightarrow}}
\def\lar{{\leftarrow}}
\def\inn{\hbox{\rm{int}}\,}
\def\sminn{\hbox{\rm \ftn{int}}\,}
\def\smql{\textrm{ql}\,}
\def\smcl{\textrm{cl}\,}
\def\smloc{\textrm{loc}\,}
\let\ftn\scriptsize


\def\ov#1{\overline{#1}}
\def\cl{\centerline}
\def\jg{J_\g}
\def\limlaw{\buildrel \DD\over\rightarrow}
\def\weaklim{\buildrel w\over\rightarrow}
\def\vaguelim{\buildrel v\over\rightarrow}
\def\eqlaw{\buildrel \DD\over =}

\def\bZ{{\mathbb Z}}
\def\bF{{\mathbb F}}
\def\bC{{\mathbb C}}
\def\bE{{\mathbb E}}
\def\bP{{\mathbb P}}
\def\bI{{\mathbb I}}
\def\bN{{\mathbb N}}
\def\bL{{\mathbb L}}
\def\bV{{\mathbb V}}


\def\Fg{{\frak g}}
\def\({\left(}
\def\){\right)}


\def\Gammab{\boldsymbol\Gamma}
\def\n{{ \boldsymbol n}}
\def\m{{\boldymbol m}}
\def\TH(#1){\label{#1}}\def\thv(#1){\ref{#1}}
\def\Eq(#1){\label{#1}}\def\eqv(#1){(\ref{#1})}
\def\diam{\hbox{\rm diam}}
\def\cov{\hbox{\rm cov}}
\def\var{\hbox{\rm var}}
\def\sfrac#1#2{{\textstyle{#1\over #2}}}

\def\bra#1{\langle #1 \rangle}
 \def\arcth{\hbox{\rm arcth}}

\let\ncl\nomenclature












